Portfolio Optimization under Nonlinear Utility

This paper studies the utility maximization problem of an agent with non-trivial endowment, and whose preferences are modeled by the maximal subsolution of a BSDE. We prove existence of an optimal trading strategy and relate our existence result to the existence of a maximal subsolution to a controlled decoupled FBSDE. Using BSDE duality, we show that the utility maximization problem can be seen as a robust control problem admitting a saddle point if the generator of the BSDE additionally satisfies a specific growth condition. We show by convex duality that any saddle point of the robust control problem agrees with a primal and a dual optimizer of the utility maximization problem, and can be characterized in terms of a BSDE solution.

==> chap05.tex <==
\section{Chapter 5}\label{sec:05}
The construction of a maximal subsolution at $t=0$ given in the previous theorem can be done for an arbitrary $t\in [0,T]$. In the next corollary we construct a subsolution which is simultaneously optimal at several points of $[0,T]$.
\begin{corollary}
\label{partition}
Let $N\in\mathbb{N}$, $N>0$. Define $\Pi^N$ the partition of $[0, T]$ given by $\Pi^N :=\{jT/2^N: j =0, \dots, 2^N \}$. Under the assumptions of Theorem \ref{existence}, there exists a triple $(\hat{X}, \hat{Y}, \hat{Z})$ which is a maximal subsolution of the system \eqref{system} at every $t \in \Pi^N$.
\end{corollary}
We will use the following easy lemma:
\begin{lemma}
Let $0\leq t_1\leq t_2\leq T$; $(X^1, Y^1, Z^1) \in \mathcal{A}_{t_1}(X^1_{t_1})$ and $(X^2, Y^2, Z^2) \in \mathcal{A}_{t_2}(X^2_{t_2})$ such that $X^1_{t_2} = X^2_{t_2}$ and $Y^1_{t_2} \leq Y^2_{t_2}$. Then putting 
\[
\bar{X} := X^11_{[t_1, t_2]} + X^21_{[t_2, T]}; \quad \bar{Y} := Y^11_{[t_1, t_2)} + Y^21_{[t_2, T]}  
\]
and
\[
\bar{Z} = Z^11_{[t_1, t_2]} + Z^21_{(t_2, T]},
\]
we have $(\bar{X}, \bar{Y}, \bar{Z}) \in \mathcal{A}_{t_1}(X^1_{t_1})$.
\end{lemma}
\begin{proof}
Let $s,t \in [0,T]$ such that $t_1 \leq s\leq t_2 \leq t \leq T$. For the backward equation, we have
\begin{align*}
&\bar{Y}_s + \int_s^tg(\bar{Y}_u, \bar{Z}_u)\,du - \int_s^t\bar{Z}_u\,dW_u\\
& = Y^1_s + \int_s^{t_2}g(Y^1_u, Z^1_u)\,du - \int_s^{t_2}Z^1_u\,dW_u + \int_{t_2}^{t}g(Y^2_u, Z^2_u)\,du - \int_{t_2}^{t}Z^2_u\,dW_u \\
&\leq Y^1_{t_2} + \int_{t_2}^{t}g(Y^2_u, Z^2_u)\,du - \int_{t_2}^{t}Z^2_u\,dW_u. \\
\end{align*}
Then by assumption 
\begin{align*}
\bar{Y}_s + \int_s^tg(\bar{Y}_u, \bar{Z}_u)\,du - \int_s^t\bar{Z}_u\,dW_u &\leq Y^2_{t_2}+ \int_{t_2}^{t}g(Y^2_u, Z^2_u)\,du - \int_{t_2}^{t}Z^2_u\,dW_u \\
&\leq Y^2_t  = \bar{Y}_t.
\end{align*}
For the forward equation, define the control process $\bar{\nu} =  \nu^11_{[t_1, t_2]} + \nu^21_{(t_2, T]}$ where $\nu^i$ is the control process associated to $X^i$; $i = 1,2$. We have
\begin{align*}
\bar{X}_{t_1} + \int_{t_1}^t\bar{\nu}_u\,dW^Q_u &= X^1_{t_1} +\int_{t_1}^{t_2}\nu^1_u\,dW_u^Q + \int_{t_2}^t\nu^2_u\,dW_u^Q\\ 
& = X^1_{t_2}  + \int_{t_2}^t\nu^2_u\,dW_u^Q\\
& = X^2_{t_2}+ \int_{t_2}^t\nu^2_u\,dW_u^Q = X^2_t = \bar{X}_t.
\end{align*}
 If $t_2 \leq s$ or $t_2 \geq t$ the result is trivial.
Therefore, $(\bar{X}, \bar{Y}, \bar{Z}) \in \mathcal{A}_{t_1}(X^1_{t_1})$.
\end{proof}
\begin{proof}[of the corollary]
For all $j = 0, \dots, 2^N$, put $t^N_j = jT/2^N$. From Theorem \ref{existence}, there exists $(\hat{X}^0, \hat{Y}^0, \hat{Z}^0)$ maximal at time $t^N_0 = 0$. Moreover, $(\hat{X}^0, \hat{Y}^0, \hat{Z}^0)\in \mathcal{A}_0(x)$ implies  $(\hat{X}^0, \hat{Y}^0, \hat{Z}^0)1_{[t^N_1, T]} \in \mathcal{A}_{t^N_1}(\hat{X}^0_{t^N_1})$. Therefore, for all $j = 1, \dots, 2^N$ there exists $(\hat{X}^j, \hat{Y}^j, \hat{Z}^j)$ in $\mathcal{A}_{t^N_j}(\hat{X}^{j-1}_{t^N_j})$ maximal at time $t^N_1$. Note that for all $j$, 
\begin{equation}
\label{arg_lem}
\hat{X}^j_{t_{j+1}^N} = \hat{X}^{j+1}_{t^N_{j+1}} \quad \text{and}\quad \hat{Y}^j_{t^N_{j+1}} \leq \hat{Y}^{j+1}_{t^N_{j+1}}.
\end{equation}
 We introduce the notation $\alpha_j:= \{t^N_0, \dots, t^N_j\}$; $j = 0, \dots, 2^N$. Put $(\hat{X}^{\alpha_0}, \hat{Y}^{\alpha_0}, \hat{Z}^{\alpha_0}) = (\hat{X}^0, \hat{Y}^0, \hat{Z}^0)$ and for $j>0$ recursively define $(\hat{X}^{\alpha_j}, \hat{Y}^{\alpha_j}, \hat{Z}^{\alpha_j})$ by 
\[
\hat{X}^{\alpha_j} = \hat{X}^{\alpha_{j-1}}1_{[0, t_j^N]} + \hat{X}^j1_{[t^N_j, T]},\quad \hat{Y}^{\alpha_j} = \hat{Y}^{\alpha_{j-1}}1_{[0, t_j^N)} + \hat{Y}^j1_{[t^N_j, T]}
\]
and 
\[
\hat{Z}^{\alpha_j} = \hat{Z}^{\alpha_{j-1}}1_{[0, t_j^N]} + \hat{Z}^j1_{(t^N_j, T]}.
\]
By the previous lemma, keeping \eqref{arg_lem} in mind, the triple $(\hat{X}^{\alpha_j}, \hat{Y}^{\alpha_j}, \hat{Z}^{\alpha_j})$ is in $\mathcal{A}_0(x)$ for each $j$. Thus, $(\hat{X}, \hat{Y}, \hat{Z}):= (\hat{X}^{\alpha_N}, \hat{Y}^{\alpha_N}, \hat{Z}^{\alpha_N}) \in \mathcal{A}_0(x)$. Let $j\in \{0,\dots, 2^N\}$. The restriction of $(\hat{X}, \hat{Y}, \hat{Z})$ on $\Omega\times [t^N_j, T]$ is in $\mathcal{A}_{t^N_j}(\hat{X}_{t^N_j}) =\mathcal{A}_{t^N_j}(\hat{X}^j_{t^N_j})$ and $\hat{Y}_{t^N_j} = \hat{Y}^j_{t^N_j}$. Hence, $(\hat{X}, \hat{Y}, \hat{Z})$ is a maximal subsolution at time $t^N_j$, which concludes the proof.
\end{proof}




==> chap06.tex <==
\subsection{Chapter 6}\label{sec:06}

